Some aspects of noise in binary classification with quantum circuits

We formally study the effects of a restricted single-qubit noise model inspired by real quantum hardware, and corruption in quantum training data, on the performance of binary classification using quantum circuits. We find that, under the assumptions made in our noise model, that the measurement of a qubit is affected only by the noises on that qubit even in the presence of entanglement. Furthermore, when fitting a binary classifier using a quantum dataset for training, we show that noise in the data can work as a regularizer, implying potential benefits from the noise in certain cases for machine learning problems.

==> arxiv_2nd <==
\begin{thebibliography}{1}

\bibitem{Arute2019}
{Arute, Frank et. al.}
\newblock Quantum supremacy using a programmable superconducting processor.
\newblock {\em Nature}, 574(7779):505--510, Oct 2019.

\bibitem{chen2014qubit}
Yu~Chen, C~Neill, Pedram Roushan, Nelson Leung, Michael Fang, Rami Barends,
  Julian Kelly, Brooks Campbell, Z~Chen, Benjamin Chiaro, et~al.
\newblock Qubit architecture with high coherence and fast tunable coupling.
\newblock {\em Physical review letters}, 113(22):220502, 2014.

\bibitem{lee2022binary}
Yonghoon Lee and Rina~Foygel Barber.
\newblock Binary classification with corrupted labels.
\newblock {\em Electronic Journal of Statistics}, 16(1):1367--1392, 2022.

\bibitem{morvan2023phase}
A.~Morvan, B.~Villalonga, X.~Mi, S.~Mandrà, A.~Bengtsson, P.~V. Klimov,
  Z.~Chen, S.~Hong, C.~Erickson, I.~K. Drozdov, J.~Chau, G.~Laun, R.~Movassagh,
  A.~Asfaw, L.~T. A.~N. Brandão, R.~Peralta, D.~Abanin, R.~Acharya, R.~Allen,
  T.~I. Andersen, K.~Anderson, M.~Ansmann, F.~Arute, K.~Arya, J.~Atalaya, J.~C.
  Bardin, A.~Bilmes, G.~Bortoli, A.~Bourassa, J.~Bovaird, L.~Brill,
  M.~Broughton, B.~B. Buckley, D.~A. Buell, T.~Burger, B.~Burkett, N.~Bushnell,
  J.~Campero, H.~S. Chang, B.~Chiaro, D.~Chik, C.~Chou, J.~Cogan, R.~Collins,
  P.~Conner, W.~Courtney, A.~L. Crook, B.~Curtin, D.~M. Debroy, A.~Del~Toro
  Barba, S.~Demura, A.~Di Paolo, A.~Dunsworth, L.~Faoro, E.~Farhi, R.~Fatemi,
  V.~S. Ferreira, L.~Flores Burgos, E.~Forati, A.~G. Fowler, B.~Foxen,
  G.~Garcia, E.~Genois, W.~Giang, C.~Gidney, D.~Gilboa, M.~Giustina, R.~Gosula,
  A.~Grajales Dau, J.~A. Gross, S.~Habegger, M.~C. Hamilton, M.~Hansen, M.~P.
  Harrigan, S.~D. Harrington, P.~Heu, M.~R. Hoffmann, T.~Huang, A.~Huff, W.~J.
  Huggins, L.~B. Ioffe, S.~V. Isakov, J.~Iveland, E.~Jeffrey, Z.~Jiang,
  C.~Jones, P.~Juhas, D.~Kafri, T.~Khattar, M.~Khezri, M.~Kieferová, S.~Kim,
  A.~Kitaev, A.~R. Klots, A.~N. Korotkov, F.~Kostritsa, J.~M. Kreikebaum,
  D.~Landhuis, P.~Laptev, K.~M. Lau, L.~Laws, J.~Lee, K.~W. Lee, Y.~D. Lensky,
  B.~J. Lester, A.~T. Lill, W.~Liu, A.~Locharla, F.~D. Malone, O.~Martin,
  S.~Martin, J.~R. McClean, M.~McEwen, K.~C. Miao, A.~Mieszala, S.~Montazeri,
  W.~Mruczkiewicz, O.~Naaman, M.~Neeley, C.~Neill, A.~Nersisyan, M.~Newman,
  J.~H. Ng, A.~Nguyen, M.~Nguyen, M.~Yuezhen Niu, T.~E. O'Brien, S.~Omonije,
  A.~Opremcak, A.~Petukhov, R.~Potter, L.~P. Pryadko, C.~Quintana, D.~M.
  Rhodes, C.~Rocque, P.~Roushan, N.~C. Rubin, N.~Saei, D.~Sank,
  K.~Sankaragomathi, K.~J. Satzinger, H.~F. Schurkus, C.~Schuster, M.~J.
  Shearn, A.~Shorter, N.~Shutty, V.~Shvarts, V.~Sivak, J.~Skruzny, W.~C. Smith,
  R.~D. Somma, G.~Sterling, D.~Strain, M.~Szalay, D.~Thor, A.~Torres, G.~Vidal,
  C.~Vollgraff Heidweiller, T.~White, B.~W.~K. Woo, C.~Xing, Z.~J. Yao, P.~Yeh,
  J.~Yoo, G.~Young, A.~Zalcman, Y.~Zhang, N.~Zhu, N.~Zobrist, E.~G. Rieffel,
  R.~Biswas, R.~Babbush, D.~Bacon, J.~Hilton, E.~Lucero, H.~Neven, A.~Megrant,
  J.~Kelly, I.~Aleiner, V.~Smelyanskiy, K.~Kechedzhi, Y.~Chen, and S.~Boixo.
\newblock Phase transition in random circuit sampling, 2023.

\bibitem{Peters2021}
Evan Peters, Jo{\~a}o Caldeira, Alan Ho, Stefan Leichenauer, Masoud Mohseni,
  Hartmut Neven, Panagiotis Spentzouris, Doug Strain, and Gabriel~N. Perdue.
\newblock Machine learning of high dimensional data on a noisy quantum
  processor.
\newblock {\em npj Quantum Information}, 7(1):161, Nov 2021.

\bibitem{reagor2016quantum}
Matthew Reagor, Wolfgang Pfaff, Christopher Axline, Reinier~W Heeres, Nissim
  Ofek, Katrina Sliwa, Eric Holland, Chen Wang, Jacob Blumoff, Kevin Chou,
  et~al.
\newblock Quantum memory with millisecond coherence in circuit qed.
\newblock {\em Physical Review B}, 94(1):014506, 2016.

\bibitem{schuld2020circuit}
Maria Schuld, Alex Bocharov, Krysta~M Svore, and Nathan Wiebe.
\newblock Circuit-centric quantum classifiers.
\newblock {\em Physical Review A}, 101(3):032308, 2020.

\bibitem{siddiqi2021engineering}
Irfan Siddiqi.
\newblock Engineering high-coherence superconducting qubits.
\newblock {\em Nature Reviews Materials}, 6(10):875--891, 2021.

\bibitem{PhysRevX.10.041038}
Yiqing Zhou, E.~Miles Stoudenmire, and Xavier Waintal.
\newblock What limits the simulation of quantum computers?
\newblock {\em Phys. Rev. X}, 10:041038, Nov 2020.

\end{thebibliography}

